Bootstrap Method in Theoretical Physics

In the realm of contemporary physics, the bootstrap method is typically associated with an optimization-based approach to problem-solving. This method leverages our understanding of a specific physical problem, which is used as the constraints for the optimization problem, to carve out the allowed region of our physical theory. Notably, this method often yields not only precise numerical bounds for physical quantities but also offers theoretical insights into the nature of the problem at hand. The modern numerical bootstrap method has seen its greatest success in the fields of conformal field theory (via the conformal bootstrap) and Scattering amplitude (through the S-matrix bootstrap). This dissertation presents the application of the bootstrap method to matrix models (random matrices), Yang-Mills theory, and conformal field theory. We will commence with a review of the fundamental elements of these theories. Following this, we will delve into the bootstrap studies of these models.

==> others/liste_publi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addchapnonumber{Liste des publications}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Articles à comité de lecture}

% Voir les macro MyprodwithDOI et Myprod dans config/macro.tex

\MyprodwithDOI{\textbf{Co Auteur 1}, Co Auteur 2, Co Auteur 3}
{Un long titre d'article}{Un journal qui a accepté mon travail}{a1b2c3d4.xxxxx.99999}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Articles en préparation}

\Myprod{\textbf{Co Auteur 1}, Co Auteur 2, Co Auteur 3}
{Le long titre de mon second article}{Le journal de mes rêves}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Conférences internationales (premier auteur)}

\Myprod{\textbf{Co Auteur 1}, Co Auteur 2, Co Auteur 3, Co Auteur 4}
{Titre de la présentation}{Conférence de Sciences, Quelque part, 2020}


